Expressiveness of Visibly Pushdown Transducers

Visibly pushdown transducers (VPTs) are visibly pushdown automata extended with outputs. They have been introduced to model transformations of nested words, i.e. words with a call/return structure. As trees and more generally hedges can be linearized into (well) nested words, VPTs are a natural formalism to express tree transformations evaluated in streaming. This paper aims at characterizing precisely the expressive power of VPTs with respect to other tree transducer models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{S. Maneth (Ed.): Workshop on Trends in Tree\\
Automata and Tree Transducers (TTATT 2013).\\
EPTCS 134, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.134.3}{10.4204/EPTCS.134.3}}

